Filaments in the southern giant lobe of Centaurus A: constraints on nature and origin from modelling and GMRT observations

We present results from imaging of the radio filaments in the southern giant lobe of Centaurus A using data from GMRT observations at 325 and 235 MHz, and outcomes from filament modelling. The observations reveal a rich filamentary structure, largely matching the morphology at 1.4 GHz. We find no clear connection of the filaments to the jet. We seek to constrain the nature and origin of the vertex and vortex filaments associated with the lobe and their role in high-energy particle acceleration. We deduce that these filaments are at most mildly overpressured with respect to the global lobe plasma showing no evidence of large-scale efficient Fermi I-type particle acceleration, and persist for ~ 2-3 Myr. We demonstrate that the dwarf galaxy KK 196 (AM 1318-444) cannot account for the features, and that surface plasma instabilities, the internal sausage mode and radiative instabilities are highly unlikely. An internal tearing instability and the kink mode are allowed within the observational and growth time constraints and could develop in parallel on different physical scales. We interpret the origin of the vertex and vortex filaments in terms of weak shocks from transonic MHD turbulence or from a moderately recent jet activity of the parent AGN, or an interplay of both.

==> journals.tex <==
\bibpunct{(}{)}{;}{a}{}{,}
\def\aap{A\&A}                % Astronomy and Astrophysics
\def\aapr{A\&A~Rev.}          % Astronomy and Astrophysics Reviews
\def\aaps{A\&AS}              % Astronomy and Astrophysics, Supplement
\def\aj{AJ}                   % Astronomical Journal
\def\ajph{Australian J.~Phys.}% Australian Journal of Physics
\def\alet{Astro.~Lett.}       % Astronomical Letters
\def\ao{Applied Optics}       % Applied Optics
\def\apj{ApJ}                 % Astrophysical Journal
\def\apjl{ApJ}                % Astrophysical Journal, Letters
\def\apjs{ApJS}              % Astrophysical Journal, Supplement
\def\apss{Ap\&SS}             % Astrophysics and Space Science
\def\araa{ARA\&A}             % Annual Review of Astronomy and Astrophysics
\def\asr{Av.~Space Res.}     % Advances in Space Research
\def\azh{AZh}                 % Astronomiceskij Zhurnal
\def\baas{BAAS}               % Bulletin of the American Astronomical Society
\def\cpc{Comput.~Phys.~Commun.} % Computer Physics Communications
\def\gca{Geochim.~Cosmochim.~Acta} % Cheochimica et Cosmochimica Acta
\def\iaucirc{IAU Circ.}       % International Astronomical Union, Circular
\def\ibvs{IBVS}               % International Bulletin of Variable Stars
\def\icarus{Icarus}           % Icarus
\def\jcomph{J.~Comput.~Phys.} % Journal of Computational Physics
\def\jcp{J.~Chem.~Phys.}      % Journal of Chemical Physics
\def\jgr{J.~Geophys.~R.}      % Journal of Geophysical Research
\def\jrasc{JRASC}             % Journal of the RAS of Canada
\def\met{Meteoritics}         % Meteoritics
\def\mmras{MmRAS}             % Memoirs of the Royal Astronomical Society
\def\mnras{MNRAS}             % Monthly Notices of the RAS
\def\mps{Meteoritics and Planetary Science} % Meteoritics and Planetary Science
\def\nast{New Astron.}        % New Astronomy
\def\nat{Nature}              % Nature
\def\pasj{PASJ}               % Publ. of the Astronomical Society of Japan
\def\pasp{PASP}               % Publ. of the Astron. Society of the Pacific
\def\phr{Phys.~Rev.}          % Physical Review
\def\pdra{Phys.~Rev.~A}       % Physical Review A
\def\prb{Phys.~Rev.~B}       % Physical Review B
\def\prc{Phys.~Rev.~C}       % Physical Review C
\def\prd{Phys.~Rev.~D}       % Physical Review D
\def\phrep{Phys.~Rep.}        % Physics Reports
\def\phss{Phys.~Stat.~Sol.}        %
\def\procspie{Proc.~SPIE}     % Proceedings of the SPIE
\def\planss{Planet.~Space Sci.}  % Planetary & Space Sciences
\def\qjras{QJRAS}             % Quarterly Journal of the RAS
\def\rpph{Rep.~Prog.~Phys.}   % Reports on Progress in Physics
\def\rgsp{Rev.~Geophys.~Space Phys.~} % Reviews on Geophysics and Space Physics
\def\sal{Soviet Astron.~Lett.}% Soviet Astronomy Letters
\def\sci{Science}             % Science
\def\solph{Sol.~Phys.}        % Solar Physics
\def\ssr{Space Sci.~Rev.}     % Space Science Reviews
\def\zap{Z.~Astrophys.}       % Zeitschrift fuer Astrophysik

